HoloSplat: Real-Time Token Streaming for Feed-Forward Human Reconstruction

Live free-viewpoint video streaming of humans enables immersive telepresence and interactive XR applications. However, this requires reconstructing each frame in real time, transmitting the data within strict bandwidth budgets, and decoding it on lightweight client GPUs. Existing approaches, whether relying on per-frame optimization or feed-forward inference, generate massive 3D Gaussian payloads that exceed practical streaming limits, while aggressive compression severely degrades rendering quality. In this work, we present HoloSplat, a real-time streaming framework for human-centric volumetric video. HoloSplat splits a feed-forward reconstructor before its Gaussian head, introducing a multi-rate streaming codec driven by server-side token compression and client-side token restoration. On the server side, we apply opacity-guided token pruning, PCA-based dimensionality reduction, and lossless geometry coding for token anchors. On the client side, a feature reconstruction hypernetwork is fused into the Gaussian head to recover compression-induced quality loss. Furthermore, we introduce Neural Session Calibration (NSC), which rapidly fine-tunes the Gaussian head online using incoming camera views during a warm-up phase. This resolves quality degradation from novel camera parameters and varying capture conditions with zero per-frame overhead. In our evaluations, HoloSplat averages 32.2 FPS on four RTX 5090 GPUs at 50 Mbit/s. It decodes each frame into 3D Gaussians in 22.1 ms on an RTX 3050 Ti laptop GPU, transmitting 22.8$\times$ less data than uncompressed float32 Gaussians, while calibrated decoding improves PSNR by 1.050 dB.

==> fig/kit/geometry.tex <==
\def\PacketAnchorKB{51.4}
\def\PacketCoefKB{270.2}
\def\PacketAnchorFrac{0.1590}
\def\PacketCoefFrac{0.8367}
\def\PacketRank{48}
\def\PacketGroups{8,038}


==> fig/teaser_plot.tex <==
\begin{axis}[hcplot, name=tpA, at={(\TPX cm,\TPY cm)}, anchor=south west, scale only axis, width=\TPW cm, height=\TPH cm, xmode=log, xmin=0.07, xmax=28.117322459463345, xtick={0.1,1,10}, xticklabels={0.1,1,10}, xminorticks=false, ymin=15.0, ymax=28.0, ytick={16,20,24,28}, xlabel={Server time (s/frame)}, xlabel style={yshift=2pt}, clip=false, x axis line style={-}, y axis line style={-}, ylabel={PSNR (dB)}, ylabel style={yshift=-5pt}]
\addplot[only marks, mark=*, mark size=2pt, mark options={draw=srv, fill=srv, line width=0.9pt}] coordinates {(2.103,17.677)};
\addplot[only marks, mark=*, mark size=2pt, mark options={draw=ses, fill=ses, line width=0.9pt}] coordinates {(1.297,15.909)};
\addplot[only marks, mark=*, mark size=2pt, mark options={draw=ink!50, fill=ink!50, line width=0.9pt}] coordinates {(2.579,23.570)};
\addplot[only marks, mark=*, mark size=2pt, mark options={draw=srv, fill=white, line width=0.9pt}] coordinates {(2.264,19.604)};
\addplot[only marks, mark=*, mark size=2pt, mark options={draw=ses, fill=white, line width=0.9pt}] coordinates {(8.653,20.672)};
\addplot[only marks, mark=*, mark size=2pt, mark options={draw=ink!50, fill=white, line width=0.9pt}] coordinates {(2.288,25.582)};
\addplot[only marks, mark=hcstar, mark size=2.8pt, mark options={draw=hot, fill=hot, line width=0.2pt}] coordinates {(0.1567,25.952) (0.1597,26.298) (0.1584,26.378)};
\node[anchor=south west, font=\sffamily\scriptsize\bfseries, text=hot, inner sep=1pt] at (axis cs:0.1285,26.68) {Ours};
\draw[->, hot, line width=0.7pt] (axis cs:0.1597,25.05) -- (axis cs:2.556,25.05);
\node[anchor=north, font=\sffamily\scriptsize\bfseries, text=hot, inner sep=1pt] at (axis cs:0.639,24.90) {\CmpDynSpeedupMean$\times$ faster};
\node[anchor=south west, font=\sffamily\scriptsize, align=left, inner sep=1pt] at (rel axis cs:0.03,0.38) {\textcolor{srv}{$\bullet$}\,HiCoM\\[-1pt]\textcolor{ses}{$\bullet$}\,QUEEN-l\\[-1pt]\textcolor{ink!50}{$\bullet$}\,3DGStream};
\end{axis}
\begin{axis}[hcplot, name=tpB, at={($(tpA.south east)+(\TPG cm,0)$)}, anchor=south west, scale only axis, width=\TPW cm, height=\TPH cm, xmode=log, xmin=0.06569003999999999, xmax=239.01201263999997, xtick={0.1,1,10,100}, xticklabels={0.1,1,10,100}, xminorticks=false, ymin=15.0, ymax=28.0, ytick={16,20,24,28}, xlabel={Payload (MB/frame)}, xlabel style={yshift=2pt}, clip=false, x axis line style={-}, y axis line style={-}, yticklabels={}]
\addplot[only marks, mark=*, mark size=2pt, mark options={draw=srv, fill=srv, line width=0.9pt}] coordinates {(3.4,17.677)};
\addplot[only marks, mark=*, mark size=2pt, mark options={draw=ses, fill=ses, line width=0.9pt}] coordinates {(53.96,15.909)};
\addplot[only marks, mark=*, mark size=2pt, mark options={draw=ink!50, fill=ink!50, line width=0.9pt}] coordinates {(8.054,23.570)};
\addplot[only marks, mark=*, mark size=2pt, mark options={draw=srv, fill=white, line width=0.9pt}] coordinates {(1.703,19.604)};
\addplot[only marks, mark=*, mark size=2pt, mark options={draw=ses, fill=white, line width=0.9pt}] coordinates {(48.46,20.672)};
\addplot[only marks, mark=*, mark size=2pt, mark options={draw=ink!50, fill=white, line width=0.9pt}] coordinates {(8.01,25.582)};
\addplot[only marks, mark=hcstar, mark size=2.8pt, mark options={draw=hot, fill=hot, line width=0.2pt}] coordinates {(0.1105,25.952) (0.2291,26.298) (0.349,26.378)};
\node[anchor=south west, font=\sffamily\scriptsize\bfseries, text=hot, inner sep=1pt] at (axis cs:0.0906,26.68) {Ours};
\node[anchor=south west, font=\sffamily\scriptsize, align=left, inner sep=1pt, text=ink!80] at (rel axis cs:0.03,0.04) {$\bullet$\,8 views\\[-1pt]$\circ$\,40 views};
\end{axis}

